Order Out of Chaos: Slowly Reversing Mean Flows Emerge from Turbulently Generated Internal Waves

We demonstrate via direct numerical simulations that a periodic, oscillating mean flow spontaneously develops from turbulently generated internal waves. We consider a minimal physical model where the fluid self-organizes in a convective layer adjacent to a stably stratified one. Internal waves are excited by turbulent convective motions, then nonlinearly interact to produce a mean flow reversing on timescales much longer than the waves' period. Our results demonstrate for the first time that the three-scale dynamics due to convection, waves, and mean flow is generic and hence can occur in many astrophysical and geophysical fluids. We discuss efforts to reproduce the mean flow in reduced models, where the turbulence is bypassed. We demonstrate that wave intermittency, resulting from the chaotic nature of convection, plays a key role in the mean-flow dynamics, which thus cannot be captured using only second-order statistics of the turbulent motions.

==> defs.tex <==

\def\red{\textcolor{red}}
\def\blue{\textcolor{blue}}
%\def\black\textcolor{black}}
\def\magenta{\textcolor{Fuchsia}}
\def\yellow{\textcolor{BurntOrange}}
\definecolor{darkblue}{RGB}{83,0,93}
\def\L{\mbox{------}}
\def\dashL{\mbox{-~-~-}}
\def\dotL{\mbox{$\cdot\cdot\cdot\cdot\cdot$}}
\def\cdashL{\mbox{---~-~---}\ :\ }
\def\cdotL{\mbox{-- $\cdot$ --}}
\def\ccdotL{\mbox{--- $\cdot\ \cdot$ ---}}
\def\longdashL{\mbox{--~--~--}}
\def\zz{($...$)\ }
\def\dashdot{\mbox{- $\cdot$ -}}

\def\bes{\begin{eqnarray}}
\def\ees{\end{eqnarray}}
\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\ba#1\ea{\begin{align}#1\end{align}}
\def\bsa#1#2\esa{\begin{subequations}\label{#1}
\begin{align}#2\end{align} \end{subequations}}
\def\lp{\left(}
\def\rp{\right)}
\def\lb{\left[}
\def\rb{\right]}
\def\lcb{\left\{}
\def\rcb{\right\}}
\def\lap{\nabla^2}
\def\g{\nabla}
\def\f{\frac}
\def\b{\mathbf}
\def\p{\partial}
\def\co{{\mathcal O}}
\def\d{\textrm d}
\def\k{{\bf{k}}}
\def\ep{\epsilon}
\def\O{\mathcal{O}}
\def\nn{\nonumber}
\DeclareMathOperator{\cotan}{cotan}


%\input{definitionsJFM}
%%\input{definitions1}
\def\u{\bm{u}}

\def\qz{\langle Q \rangle_z}
\def\NA{\bm{\nabla}}
\def\DEL{\nabla^2}
\def\mt{\overline{\langle T \rangle}_x}
\def\mr{\overline{\langle \rho \rangle}_x}
\def\Nu{\text{Nu}}
\def\Ra{\text{Ra}}
\def\Pr{\text{Pr}}
\def\s{\text{S}}
\def\Z{Z_{\text{NB}}}

\def\blue{\textcolor{blue}}

